Weighted Information Filtering, Smoothing, and Out-of-Sequence Measurement Processing

We consider the problem of state estimation in dynamical systems and propose a different mechanism for handling unmodeled system uncertainties. Instead of injecting random process noise, we assign different weights to measurements so that more recent measurements are assigned more weight. A specific choice of exponentially decaying weight function results in an algorithm with essentially the same recursive structure as the Kalman filter. It differs, however, in the manner in which old and new data are combined. While in the classical KF, the uncertainty associated with the previous estimate is inflated by adding the process noise covariance, in the present case, the uncertainty inflation is done by multiplying the previous covariance matrix by an exponential factor. This difference allows us to solve a larger variety of problems using essentially the same algorithm. We thus propose a unified and optimal, in the least-squares sense, method for filtering, prediction, smoothing and general out-of-sequence updates. All of these tasks require different Kalman-like algorithms when addressed in the classical manner.

==> abstract.tex <==
\begin{abstract}
We propose a deterministic framework for state estimation in dynamical systems. As opposed to the classical Bayesian approach, where (random) process noise is used to cope with inevitable uncertainties in the dynamical model, in the proposed modeling, this uncertainty is treated by assigning exponentially decaying weights to the observations, such that more recent measurements are assigned more weight than ``older'' ones. The state is then estimated using a weighted least-squares (WLS) algorithm as opposed to Bayesian methods such as, e.g., Kalman filter. For the chosen weighting function, the least squares algorithm possesses a convenient recursive form similarly to the Kalman filter. Both the deterministic formulation and the exponential weighting have been addressed, separately, in the literature in the past. Introducing the latter into the deterministic framework is novel and, in the absence of process noise, allows exact solutions to problems which may be solved only approximately  in the Bayesian setup. In this paper we concentrate on out-of-sequence measurement (OOSM) processing which is one of such problems. We develop a unified, optimal, in the WLS sense, algorithm for filtering and smoothing in dynamical systems in the presence of OOSM.

\end{abstract}


\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\section{Introduction}\label{section:intro}
State estimation in dynamical systems has become a topic of active research since the publication of Rudolf Kalman's study in 1960. In Kalman's setup an unknown state sequence is modeled as a stochastic process evolving through a linear system and driven by an external random process noise. The sequence is observed by a linear measurement channel contaminated by random measurement noits. The resulting Kalman filter (KF) is an optimal, in the minimum mean-square error (MMSE) sense, recursive algorithm for the estimation of the state using the available measurements. Numerous generalizations and modifications to the basic version of KF have been proposed. Optimal prediction and smoothing algorithms~\cite{anderson1979optimal} are only two examples. A more recent notion of out-of-sequence measurement (OOSM) processing has become popular since the publication~\cite{ybs:2002:oosm}. In these and other cases a modification to the classical KF algorithm was proposed and a different algorithm was derived. In some cases, such as Kalman smoothing and one-step OOSM~\cite{ybs:2002:oosm}, the algorithms remain optimal. There are scenarios, however, in which preserving optimality is no longer possible. The problem of multi-step OOSM processing~\cite{ybs:2004:oosm:multistep} is a good example of such scenario. Typically, the hardness in the derivation of an algorithm or in maintaining its optimality is rooted in the correlations generated by the process noise sequence and earlier measurements. On the other hand, the process noise is an inevitable mechanism in order to treat mismatches in the dynamical model of the state sequence.

In this paper we propose a deterministic formulation of the state sequence without process noise. Consequently, a weighted least-squares algorithm may be used to compute the estimates of the state. Instead of a random process noise it is suggested to assign weights to different components of the WLS cost such that older measurements contribute less than new ones. Choosing a convenient special case of exponentially decaying weight function it is possible to derive a recursive version of the optimal WLS algorithm. Due to the absence of the process noise, the algorithm implements unified measurement updates for different problems and, on the other hand, preserves optimality.
Therefore, we propose an optimal, recursive, universal method for state estimation under a variety of measurement configurations.
This method allows the computation of state estimates in a variety of problems using a single optimal algorithm.


The remainder of the paper is organized as follows. In Section~\ref{section:problem} we formally state the problem at hand and list the relevant assumptions. Section~\ref{section:derivation} is devoted to the derivation of several algorithms starting with the simplest case of a batch-type estimator and proceeding to more complex, recursive routines. In Section~\ref{section:properties:examples} several important properties of the derived estimator are discussed and some illustrative simple examples are provided. In Section~\ref{section:wif} we consider an important special cases of the general algorithm and compare it with the classical KF. In Section~\ref{section:applications} several applications are considered the main of which is OOSM processing in the filtering and smoothing framework. Concluding remarks are given in Section~\ref{section:concluding}.



\section{Problem Setup}\label{section:problem}
We consider a dynamical system evolving between discrete time-instances $t_1,t_2,\ldots,t_k$ such that $t_k$ represents the $k$-th sampling time. The evolution of the system is captured by the following \emph{deterministic} equation
\begin{align}\label{Eq:problem:state}
x_k = A_{k,\ell}x_\ell+C_{k,\ell}u_{k,\ell},
\end{align}
where $x_k$ is the system state at time $t_k$, $A_{k,\ell}$ is the known state transition matrix from time $t_\ell$ to time $t_k$ and $u_{k,\ell}$ is the cumulative effect of the deterministic inputs applied during the time interval $(t_\ell,t_k]$. The initial state $x_0$ is assumed to be deterministic but unknown. We emphasize that we do not assume that the system is driven by a (random) process noise meaning that the only uncertainty in the described system is the initial state $x_0$. In other words, no probabilistic modeling is associated with the sequence $\set{x_k}$. For all $k,\ell\in\mathbb{N}$, the matrices $\set{A_{k,\ell}}$  are assumed to be invertible~\cite{ybs:2002:oosm}. Similarly to~\eqref{Eq:problem:state}, assuming appropriate controllability conditions, we may express $x_\ell$, for all $\ell$, using $x_k$ as follows
\begin{align}\label{Eq:problem:state:reverse}
x_\ell = A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k}.
\end{align}
The state is observed through the following linear Gaussian measurement channel
\begin{align}\label{Eq:problem:measurement}
y_\ell = H_\ell x_\ell+v_{\ell},
\end{align}
where $H_\ell$ is a known matrix, and $\set{v_\ell}$ is a sequence of independent Gaussian random variables such that $v_\ell\sim\gaus{0}{R_\ell}$.


Our goal is the estimation of the state $x_k$ using the available measurements $\set{y_\ell,\,\ell\in\mathcal{L}}$  for some set of indices $\mathcal{L}$. Note that since the state sequence is deterministic, every measurement in the set $\mathcal{L}$ may be viewed as a measurement of $x_k$ without adding uncertainty (in addition to the measurement noise $v_\ell$). This is different from the Bayesian setup in which, in addition to the measurement noise, there is additional uncertainty due to the contribution of the process noise in the time interval defined by the considered measurement and the desired state $x_k$. In the absence of a probabilistic prior for $x_k$, and taking into account the symmetry of the distribution of $v_k$, we utilize the relation~\eqref{Eq:problem:state:reverse} and consider the following weighted least-squares (WLS) cost
\begin{align}\nonumber
&\operatorname{argmin}_{x_k}\sum_{\ell\in\mathcal{L}}(H_\ell(A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k})-y_\ell)^T\\\label{Eq:problem:WLS}
&\qquad \times W_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(H_\ell(A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k})-y_\ell).
\end{align}
The weighting matrix of the $\ell$-th element in the above comprises two elements -- the inverse covariance matrix of the corresponding measurement noise and an additional matrix $W_{\ell,k}$ which will play a crucial role in the sequel. Intuitively, the dependence of $W_{\ell,k}$ on $k$ causes this matrix to account for the relevance of the distant measurement $y_\ell$ for the estimation of the present state $x_k$.
%Note that if we drop the dependence of $W_{\ell,k}$ on $k$ and replace the weighting matrix with an arbitrary one, $W_{\ell}$, that %depends only on the time of the measurement $y_\ell$, it will be equivalent to defining the measurement equation~\eqref{Eq:problem:measurement} in the following way
Note that the problem~\eqref{Eq:problem:WLS} could be obtained by using the following formulation of the measurement equation for some index $k$,
\begin{align}\label{Eq:problem:measurement2}
y_\ell = H_\ell x_\ell+\tilde{W}_{\ell,k}v_{\ell},
\end{align}
where $\tilde{W}_{\ell,k}={W}_{\ell,k}^{-T}$ and the effective measurement noise covariance
\begin{align}\label{Eq:problem:measurement2:covariance}
\EE{\tilde{W}_{\ell,k}v_{\ell}v_\ell^T\tilde{W}_{\ell,k}^T}
    =\tilde{W}_{\ell,k}R_\ell\tilde{W}_{\ell,k}^T
    ={W}_{\ell,k}^{-T}R_\ell{W}_{\ell,k}^{-1}.
\end{align}
For this setup,~\eqref{Eq:problem:WLS} is a standard WLS cost with optimal weights meaning its solution is the best linear unbiased estimator (BLUE).

In the following section we derive optimal, in the sense of Eq.~\ref{Eq:problem:WLS}, estimator and consider special cases in which recursive formulation of the estimator is possible.

\section{Derivation of the Estimator}\label{section:derivation}
\subsection{Batch-Form Estimator}\label{section:batch:derivation}
We begin with the derivation of the optimal estimator, in batch form, for the quadratic cost~\eqref{Eq:problem:WLS}. For clarity of the exposition we consider~\eqref{Eq:problem:measurement2} as the measurement model. The first result, which is a straightforward generalization of the classical LS solution, is summarized in the following two Theorems.
\begin{theo}\label{theorem:batch}
Let $\set{y_\ell,\,\ell\in\mathcal{ L}}$ be a general set of measurements defined in~\eqref{Eq:problem:measurement2}. The optimal solution of the problem~\eqref{Eq:problem:WLS} subject to the constraint~\eqref{Eq:problem:state} is
\begin{align}\non
\hat{x}_k
&=\paren{\sum_{\ell\in\mathcal{L}}A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^TH_\ell A_{\ell,k}}^{-1}\\\label{Eq:batch:estimator}
&\qquad\times\sum_{\ell\in\mathcal{L}}A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(y_\ell-H_\ell C_{\ell,k}u_{\ell,k}).
\end{align}
\end{theo}
\begin{proof} See Appendix~\ref{appendix:batch}.
\end{proof}

\begin{theo}\label{theorem:covariance}
The covariance of the estimator~\eqref{Eq:batch:estimator} is given by
\begin{align}\non
P_k&\triangleq\EE{(\hat{x}_k-\EE{\hat{x}_k})(\hat{x}_k-\EE{\hat{x}_k})^T}\\\label{Eq:batch:covariance}
&=\paren{\sum_{\ell\in\mathcal{L}}A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell}^TH_\ell A_{\ell,k}}^{-1}.
\end{align}
\end{theo}
\begin{proof} See Appendix~\ref{appendix:covariance}.
\end{proof}
Theorem~\ref{theorem:covariance} allows us to rewrite~\eqref{Eq:batch:estimator} in the following compact form
\begin{align}\label{Eq:batch:estimator:compact}
\hat{x}_k=P_k\sum_{\ell\in\mathcal{L}}A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(y_\ell-H_\ell C_{\ell,k}u_{\ell,k}).
\end{align}

For notational convenience and without loss of generality, in the sequel, we set $u_{\ell,k}=0$ for all $k\in\mathbb{N}$ and $\ell\in\mathcal{L}$.

\subsection{Recursive Estimator}\label{section:derivation:recursive}
We now consider a narrower family of the weighting matrices $W_{\ell,k}$ that depend explicitly both on the time of the currently considered measurement $y_\ell$, and on the time of the state to be estimated $x_k$, thus accounting for the relevance of $y_\ell$ on the estimation of $x_k$. As we show in the sequel, this family allows recursive computation of the estimator~\eqref{Eq:batch:estimator} and the corresponding covariance~\eqref{Eq:batch:covariance}.

We still consider the measurement model~\eqref{Eq:problem:measurement2} which we rewrite here for convenience
\begin{align}\label{Eq:problem:measurement3}
y_\ell = H_\ell x_\ell+\tilde{W}_{\ell,k}v_{\ell}.
\end{align}
%The idea is to allow the weighting matrix to depend both on the time of the distant measurement $y_\ell$ and on the time of the desired state $x_k$, thus accounting for the relevance of $y_\ell$ on the estimation of $x_k$.
The weight assigned to $y_\ell$ reduces as the difference ${t_k-t_\ell}$ increases. In this work we take $W_{\ell,k}$ to be a scalar-valued function with the following properties: %
\begin{subequations}\label{Eq:recursive:W:properties}
\begin{align}\label{Eq:recursive:W:positive}
W_{\ell,k}&\geq0, \forall\ \ell, k\\\label{Eq:recursive:W:equal}
W_{k,k}&=1\\\label{Eq:recursive:W:telescopic}
%W_{\ell,k}&=W_{k-1,k}W_{\ell,k-1}.
W_{\ell,k}&=W_{\ell,m}W_{m,k}.
\end{align}
\end{subequations}
A simple example of such a function, to be used extensively in the sequel, is
\begin{align}\label{Eq:recursive:W}
W_{\ell,k} = e^{-{(t_k-t_\ell)}/2\tau},\quad\tau>0.
\end{align}
Informally, the parameter $\tau$ may be viewed as a ``weight decay factor'' or as a ``decorrelation interval'' such that the amount of information about the state, stored in the measurements, reduces as the temporal distance between these measurements and the state increases.

The main results of the paper are now stated in the following three Theorems.
\begin{theo}\label{theorem:recursive}
Let $\mathcal{L}=\set{1,2,\ldots,k}$. The estimator~\eqref{Eq:batch:estimator} with the weighting matrix~\eqref{Eq:recursive:W:properties} may be computed recursively as follows
%\begin{align}\label{Eq:recursive:estimator}
%\hat{x}_k=P_k\paren{e^{-\frac{t_k-t_{k-1}}{2\tau}}A_{k-1,k}^TP_{k-1}^{-1}(\hat{x}_{k-1}-u_{k-1,k})+H_k^TR_k^{-1}y_k},
%\end{align}
%where $P_k$ is given by
%\begin{align}\label{Eq:recursive:covariance}
%P_k^{-1}={e^{-\frac{t_k-t_{k-1}}{2\tau}}A_{k-1,k}^TP_{k-1}^{-1}A_{k-1,k}+H_k^TR_k^{-1}H_k}.
%\end{align}
\begin{align}\label{Eq:recursive:estimator}
\hat{x}_k
&=P_k\big(W_{k-1,k}^2A_{k-1,k}^TP_{k-1}^{-1}\hat{x}_{k-1}+H_k^TR_k^{-1}y_k\big),
\end{align}
where the estimator covariance, $P_k$, is given by
\begin{align}\label{Eq:recursive:covariance}
P_k^{-1}={W_{k-1,k}^2A_{k-1,k}^TP_{k-1}^{-1}A_{k-1,k}+H_k^TR_k^{-1}H_k}.
\end{align}
\end{theo}
\begin{proof} See Appendix~\ref{appendix:recursive}.
\end{proof}

The setup of Theorem~\ref{theorem:recursive} implied that the measurements $\set{y_\ell,\ell\in\mathcal{L}}$ arrive sequentially, such that $y_k$ is the measurement arriving at time $t_k$ thus being an observation of the state $x_k$ according to~\eqref{Eq:problem:measurement}. We show next that this does not have to be the case. To this end, we consider a more general set of indices
\begin{align}\label{Eq:indices:new}
\mathcal{L}=\set{\ell_1,\ell_2,\ldots,\ell_k},
\end{align}
such that the measurement $y_{\ell_k}$ arrives at time $t_k$, but corresponds to time $t_{\ell_k}$. Clearly, if $\ell_k=k$ for all $\ell_k\in\mathcal{L}$, the present setup reduces to the one discussed in Theorem~\ref{theorem:recursive}.

\begin{theo}\label{theorem:recursive:general}
Let $\mathcal{L}$ be as defined in~\eqref{Eq:indices:new} and let $d$ denote the $k$-th index in $\mathcal{L}$ such that $t_d=t_{\ell_k}$. The estimator~\eqref{Eq:batch:estimator} with the weighting matrix~\eqref{Eq:recursive:W:properties} may be computed recursively as follows
\begin{align}\label{Eq:recursive:estimator:d}
\hat{x}_k
&=P_k\big(W_{k-1,k}^2A_{k-1,k}^TP_{k-1}^{-1}\hat{x}_{k-1}
+W_{d,k}^2A_{d,k}^TH_d^TR_d^{-1}y_{d}\big),
\end{align}
where the estimator covariance, $P_k$, is given by
\begin{align}\label{Eq:recursive:covariance:d}
P_k^{-1}
&=W_{k-1,k}^2A_{k-1,k}^TP_{k-1}^{-1}A_{k-1,k}+W_{d,k}^2A_{d,k}^TH_d^TR_d^{-1}H_dA_{d,k}.
\end{align}
\end{theo}
\begin{proof} The proof is along the lines of that of Theorem~\ref{theorem:recursive}.
\end{proof}
It is important to emphasize the implications of Theorem~\ref{theorem:recursive:general}. The optimal update of the estimator is not affected by the times at which the measurements are acquired, as long as the actual validity time of these measurements is known. This means that seemingly different problems such as filtering, fixed lag-smoothing, and out-of-sequence measurement processing may be treated in essentially the same manner using Eq.~\ref{Eq:recursive:estimator:d}. For example, measurements arriving out-of-sequence are optimally processed using the same algorithm as those arriving in-sequence. This is not the case in the Bayesian setup, where a different algorithm is required to incorporate OOSM. Similar argument holds for the problem of fixed-lag smoothing in which Bayesian measurement processing requires a modified algorithm (fixed-lag smoother) and cannot be done using a standard Kalman filter. Moreover, except for some special cases, OOSM processing in the Bayesian setup is either suboptimal or requires increased computational resources. On the contrary, in the discussed setting, OOSM processing remains optimal in the sense of Theorem~\ref{theorem:recursive:general}.

Inspecting the filter equations of Theorem~\ref{theorem:recursive:general} we notice that additional generalization is in place. The first summand in both~\eqref{Eq:recursive:estimator:d} and~\eqref{Eq:recursive:covariance:d} stands for the contribution of the previously updated estimate to the current time. However, the time index $k$ must not necessarily refer to some previous time and may, in fact, refer to any time in the past, present, or future. We thus may rewrite the equations of the presented algorithm such that, in addition to the ``measurement update step'' defined by the second summand in~\eqref{Eq:recursive:estimator:d} and~\eqref{Eq:recursive:covariance:d} that allows arbitrary measurement timing, the ``time propagation step'' is also arbitrary as summarized in the following Theorem.
\begin{theo}\label{theorem:recursive:general:extra}
Let $\mathcal{L}$ be as defined in~\eqref{Eq:indices:new} and let $d$ denote the $k$-th index in $\mathcal{L}$ such that $t_d=t_{\ell_k}$. In addition, let $m$ refer to an arbitrary index representing time instance $t_m$ at which $\hat{x}_m$ and $P_m$ are known.
The estimator~\eqref{Eq:batch:estimator} with the weighting matrix~\eqref{Eq:recursive:W:properties} may be computed recursively as follows
\begin{align}\label{Eq:recursive:estimator:d:extra}
\hat{x}_k
&=P_k\big(W_{m,k}^2A_{m,k}^TP_{m}^{-1}\hat{x}_{m}
+W_{d,k}^2A_{d,k}^TH_d^TR_d^{-1}y_{d}\big),
\end{align}
where the estimator covariance, $P_k$, is given by
\begin{align}\label{Eq:recursive:covariance:d:extra}
P_k^{-1}
&=W_{m,k}^2A_{m,k}^TP_{m}^{-1}A_{m,k}+W_{d,k}^2A_{d,k}^TH_d^TR_d^{-1}H_dA_{d,k}.
\end{align}
\end{theo}
\begin{proof} The proof is along the lines of that of Theorem~\ref{theorem:recursive}.
\end{proof}
Clearly, Theorem~\ref{theorem:recursive:general:extra} generalizes both Theorem~\ref{theorem:recursive} and Theorem~\ref{theorem:recursive:general} which follow as special cases.

\section{Properties and Examples}\label{section:properties:examples}

\subsection{Examples}\label{section:examples1}
\subsubsection{Static Parameter}\label{section:examples1:static}
Let $A_{k,\ell}=I$ %and $u_{k,\ell}=0$ for all $k\in\mathbb{N}$ and $\ell\in\mathcal{L}$
meaning that $x_k=x_{k-1}=\ldots=x_0$. In this case~\eqref{Eq:problem:WLS} reads
\begin{align}\label{Eq:example:WLS:static}
\arg\min_{x_k}\sum_{\ell\in\mathcal{L}}(H_\ell x_k-y_\ell)^T W_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(H_\ell x_k-y_\ell).
\end{align}
We assign equal weights to all measurements in the set $\mathcal{L}$ by setting, for all $\ell,k$, $W_{\ell,k}=1$ and obtain the following form of the estimator~\eqref{Eq:batch:estimator}:
\begin{align}\label{Eq:example:estimator:constant}
\hat{x}_k&=P_k\sum_{\ell\in\mathcal{L}}H_\ell^TR_\ell^{-1}y_\ell,
\end{align}
where the covariance, $P_k$, is given by
\begin{align}\label{Eq:example:covariance:constant}
P_k&=\paren{\sum_{\ell\in\mathcal{L}}H_\ell^TR_\ell^{-1}H_\ell}^{-1}.
\end{align}
%%%% The latter is a standard result TBD.\\
Note that $W_{\ell,k}=1$ satisfies the set of properties~\eqref{Eq:recursive:W:properties}. The corresponding recursive form of the estimator thus reads
\begin{align}\label{Eq:example:estimator:recursive:constant}
\hat{x}_k&=P_k(P_{k-1}^{-1}\hat{x}_{k-1}+H_k^TR_k^{-1}y_k)\\
P_k^{-1}&=P_{k-1}^{-1}+H_k^TR_k^{-1}H_k.
\end{align}

\subsubsection{Constant Acceleration Model}\label{section:examples1:polynomial}
Consider next a state comprising position, velocity and acceleration data such that
\[
x_0
\triangleq\begin{pmatrix}{\rm pos}_0 & {\rm vel}_0 & {\rm acc}_0\end{pmatrix}^T.
\]
%and $u_{k,\ell}=0$ for all $k\in\mathbb{N}$ and $\ell\in\mathcal{L}$.
The state evolves according to a constant acceleration (CA) model
\begin{align}\non
x_k
&=
\begin{pmatrix}1 & \Delta t & \Delta t^2/2\\0 & 1 & \Delta t\\ 0 & 0 & 1\end{pmatrix}
\begin{pmatrix}{\rm pos}_{k-1}\\{\rm vel}_{k-1}\\{\rm acc}_{k-1}\end{pmatrix}\\\label{Eq:example:WLS:CA}
&=
\begin{pmatrix}1 & t_k & t_k^2/2\\0 & 1 & t_k\\ 0 & 0 & 1\end{pmatrix}
x_0
,
\end{align}
where $\Delta t\triangleq t_k-t_{k-1}$ with only the position being observed
\[
H_k=[1\ 0\ 0].
\]
Assuming the measurement noise variance is constant and taking, as before, $W_{\ell,k}=1$,~\eqref{Eq:batch:estimator} reduces to
\begin{align}\non
\hat{x}_k
&=
\begin{pmatrix}
\sum_\ell  t_\ell^0           & \sum_\ell t_\ell              & \frac{1}{2}\sum_\ell t_\ell^2\\
\sum_\ell t_\ell              & \sum_\ell t_\ell^2 & \frac{1}{2}\sum_\ell t_\ell^3\\
\frac{1}{2}\sum_\ell t_\ell^2 & \frac{1}{2}\sum_\ell t_\ell^3 & \frac{1}{4}\sum_\ell t_\ell^4
\end{pmatrix}^{-1}
\begin{pmatrix}
\sum_\ell t_\ell^0 y_\ell\\\sum_\ell t_\ell y_\ell\\\frac{1}{2}\sum_\ell t_\ell^2 y_\ell
\end{pmatrix},
\end{align}
which is, up to the constants, is exactly the Savitzky-Golay filter~\cite{savitzky1964smoothing} for polynomial smoothing of noisy data. This observation allows us to relate Savitzki-Golay filters to the more general KF framework. In other words, polynomial smoothing can be formulated within a state-space model using appropriate transition matrix~\eqref{Eq:problem:state}, and measurement geometry~\eqref{Eq:problem:measurement}.


\subsection{Properties}\label{section:properties}
We now state several properties satisfied by the batch and recursive versions of the estimator.
\begin{theo}\label{theorem:efficient}
The estimator~\eqref{Eq:batch:estimator} is unbiased and the corresponding error covariance~\eqref{Eq:batch:covariance} attains the Cram\'{e}r-Rao lower bound with equality rendering the estimator efficient.
\end{theo}
\begin{proof} See Appendix~\ref{appendix:efficient}.
\end{proof}

\begin{lemm}\label{lemma:scaling} The optimal estimator in either batch~\eqref{Eq:batch:estimator}, or recursive~\eqref{Eq:recursive:estimator} form does not depend on the scaling of the measurement noise covariance.
\end{lemm}
\begin{proof} See Appendix~\ref{appendix:scaling}.
\end{proof}
Lemma~\ref{lemma:scaling} states that knowing the measurement noise variance is only required up to a multiplicative constant. In other words, for a constant variance of the measurement noise one does not need to tune the corresponding parameter in the filter. This desired property is only possible due to the lack of the process noise and does not happen in, e.g., Kalman-filter based algorithms.


\section{Exponentially Weighted Information Filtering}\label{section:wif}
\subsection{Concept}\label{section:wif:concept}
In this section we consider a specific function $W_{\ell,k}$ and discuss the resulting estimator. The function under consideration is~\eqref{Eq:recursive:W} which is repeated here for convenience.
\begin{align}\label{Eq:recursive:W2}
W_{\ell,k} = e^{-{(t_k-t_\ell)}/2\tau},\quad\tau>0.
\end{align}
%The weight assigned to $y_\ell$ decays exponentially as the interval $t_k-t_\ell$ increases.
It is readily seen that this weighting function satisfies the set of properties~\eqref{Eq:recursive:W:properties} such that a recursive form of the estimator~\eqref{Eq:batch:estimator} is given by~\eqref{Eq:recursive:estimator}. From this point on, however, we drop the formulation~\eqref{Eq:problem:measurement2} and return to the original setup~\eqref{Eq:problem:measurement}. Note that this does not affect the optimality of the solution in the weighted least-squares sense~\eqref{Eq:problem:WLS}. For this choice of $W_{\ell,k}$ the recursive estimator~\eqref{Eq:recursive:estimator}  takes the following form
%\begin{align}\non
%\hat{x}_k
%&=P_k\big(e^{-\frac{t_k-t_{k-1}}{\tau}}A_{k-1,k}^TP_{k-1}^{-1}(\hat{x}_{k-1}-C_{k-1,k}u_{k-1,k})\\\label{Eq:recursive:estimator:wif}
%&\qquad\qquad+H_k^TR_k^{-1}y_k\big),
%\end{align}
\begin{align}\label{Eq:recursive:estimator:wif}
\hat{x}_k
&=P_k\big(e^{-\frac{t_k-t_{k-1}}{\tau}}A_{k-1,k}^TP_{k-1}^{-1}\hat{x}_{k-1}+H_k^TR_k^{-1}y_k\big),
\end{align}
where $P_k$ is given by
\begin{align}\label{Eq:recursive:covariance:wif}
P_k^{-1}=e^{-\frac{t_k-t_{k-1}}{\tau}}A_{k-1,k}^TP_{k-1}^{-1}A_{k-1,k}+H_k^TR_k^{-1}H_k.
\end{align}
Hereafter, we term the above estimator Exponentially Weighted Information Filter (EWIF). Note that once we have dropped the formulation~\eqref{Eq:problem:measurement2}, $P_k$ given in~\eqref{Eq:recursive:covariance:wif} is no longer the covariance of the estimator, but, rather, an approximation. This is similar to a KF setup in which the model is not known precisely and an artificial process noise is used to compensate this mismatch, such the \emph{computed} covariance is not the true error covariance.

It is readily seen that if $\tau\to\infty$, $e^{-\frac{t_k-t_{k-1}}{\tau}}\to1$ and the dependence of $\hat{x}_k$ on the measurement history becomes uniform such that no extra weight is assigned to the more recent measurements. In this extreme regime the algorithm reduces to a standard KF with no process noise as we discuss in the sequel. On the contrary, when  $\tau\to0$, $e^{-\frac{t_k-t_{k-1}}{\tau}}\to0$ and $\hat{x}_k$ depends, for each $k$, solely on the current measurement $y_k$. This is similar to setting a very large process noise in the standard KF setup.

We note in passing that although exponential weighting have been addressed in the literature in the past~\cite{anderson1973exponential,anderson1979optimal}, this was never done as an approach to deterministically cope with model uncertainties. Thus, the setup considered in the present section is a novel approach to address state estimation problems under possible model mismatch.

%YYY Although exponential weighting\cite{anderson1973exponential,anderson1979optimal} have been used in the past, in this sequel we are using it as an alternative to process noise, as the dynamical property of our model. in other words, we proposing a different model for dynamic targets that have more convenient properties for estimations SSS.

\subsection{Relation to Kalman Filter}\label{section:wif:kalman}
In order to gain additional insight on the differences between the EWIF approach and a standard KF setup we consider the information form of the latter.
%\begin{align}\non
%\hat{x}_k
%&=P_k\big(A_{k-1,k}^T(P_{k-1}+Q_{k-1,k})^{-1}(\hat{x}_{k-1}-C_{k-1,k}u_{k-1,k})\\\label{Eq:information:kf:state}
%&\qquad\qquad+H_k^TR_k^{-1}y_k\big),
%\end{align}
\begin{align}\label{Eq:information:kf:state}
\hat{x}_k
&=P_k\big(A_{k-1,k}^T(P_{k-1}+A_{k-1,k}Q_{k-1,k}A_{k-1,k}^T)^{-1}\hat{x}_{k-1}+H_k^TR_k^{-1}y_k\big),
\end{align}
where $P_k$ is given by
\begin{align}\label{Eq:information:kf:covariance}
P_k^{-1}=A_{k-1,k}^T(P_{k-1}+A_{k-1,k}Q_{k-1,k}A_{k-1,k}^T)^{-1}A_{k-1,k}+H_k^TR_k^{-1}H_k.
\end{align}
Comparing~\eqref{Eq:information:kf:state} and ~\eqref{Eq:information:kf:covariance} with, respectively,~\eqref{Eq:recursive:estimator:wif} and~\eqref{Eq:recursive:covariance:wif} we make the following observations.
It is readily seen that setting $\tau\to\infty$ in~\eqref{Eq:recursive:estimator:wif} and~\eqref{Eq:recursive:covariance:wif}, and $Q_{k-1,k}=0$ in~\eqref{Eq:information:kf:state} and ~\eqref{Eq:information:kf:covariance} renders both algorithms identical.

Further, in both cases, the algorithms linearly combine two types of data -- historical information, captured by the previously obtained estimate $\hat{x}_{k-1}$, and new information stored in the currently acquired measurement $y_k$. In the KF case, the weight assigned to the history is controlled by the quantity $(P_{k-1}+A_{k-1,k}Q_{k-1,k}A_{k-1,k}^T)^{-1}$ which is the information (inverse of the covariance) associated with older measurements. The reduction in the information, relatively to $P_{k-1}^{-1}$ from step $k-1$, is dictated by the process noise covariance $Q_{k-1,k}$ such that in the case of a very unpredictable state sequence (large process noise), much uncertainty is added between two consecutive measurement updates and the amount of information stored in the previous measurements reduces. On the contrary, at the absence of process noise, the weight assigned to the history of the measurements in the EWIF approach is controlled by the quantity $e^{-\frac{t_k-t_{k-1}}{\tau}}P_{k-1}^{-1}$. Since for $t_k\geq t_{k-1},\tau\geq0$,
\[
e^{-\frac{t_k-t_{k-1}}{\tau}}\leq1,
\]
the information associated with the measurement history reduces similarly to the KF case. In other words, the difference between the KF-based approach and the proposed EWIF method boils down to the method the contribution of historical measurements is managed -- additive increase of the error covariance in the case of KF versus multiplicative inflation of the covariance in EWIF.

Our final comment is on the specific information reduction mechanism. While in the standard KF setup the weight assigned to the measurement history is controlled by the state process noise or, equivalently, by our assumptions on the system predictability, in the proposed approach this weight control mechanism is completely decoupled from the state and only considers the measurement sequence. This observation gains the EWIF approach additional robustness to the state process model mismatch similarly to the Savitzky-Golay filter. The parameter $\tau$ becomes then nothing more than a tuning parameter as opposed to the Bayesian case where the process noise covariance has to be carefully chosen for each state dynamics based on some prior knowledge.

%YYYIn fact, in the EWIF case the motivation and the meaning of the reduction in information can be much clearer, while the KF have to guess the process noise of the target, in the EWIF case the coefficient $\tau$ is not a guess or a property of the target, it is a property of 'how smooth the user wants its estimation'. In other words, the EWIF is much more robust for different types of target properties, similarly to Savitzky-Golay filter. SSS DS NEED TO THINK AGAIN - KF DPES NOT NEED TO KNOW Q - IT IS ONLY A TUNING PARAMETER SD

\subsection{Toy Example}\label{section:wif:toy}
We now demonstrate the utility of the EWIF approach in a simple synthetic example. We consider a one-dimensional sinusoidal signal observed by a sequence of linear measurements corrupted by zero-mean Gaussian noise with covariance $0.5$.
Note that the state at $k+1$ cannot be described by as linear transformation of the state at $k$. Thus, in order to track the sequence with a \emph{linear} filter one has to compensate the model mismatch. We estimate the sequence of states using a linear Kalman filter in which the model mismatch is compensated by a process noise such that the state equation is
\[
x_k=x_{k-1}+w_k,
\]
where $\set{w_k}$ is a zero-mean white process noise sequence with standard deviation $\sigma_w=0.1$. Alternatively, the states are tracked using the EWIF algorithm with decorrelation constant $\tau=0.5$. The resulting estimates are presented in Fig.~\ref{fig:toy:sine}.
\begin{figure}[h!]\centering
{\includegraphics[width=0.75\columnwidth, trim=0cm -0.5cm 0cm 0cm, clip]{fig1_0_new.eps}}%\hspace{0.2cm}
\caption{The performance of EWIF (green) and KF (magenta) in a simple example of tracking a sine signal. The two estimated sequences are practically indistinguishable -- the RMS errors of EWIF and KF are $0.31$ and $0.33$, respectively.}
\label{fig:toy:sine}
\end{figure}
It is readily seen that, for the described parameter setup, both algorithms achieve similar performance. This demonstrates the history handling mechanism carried out by the two methods as discussed in Section~\ref{section:wif:kalman} and also suggests that, in similar estimation problems, for a given value of $\sigma_w$, one can find an ``equivalent'' value of $\tau$.

%\subsection{Discussion}\label{section:wif:discussion}
%\begin{enumerate}
%  \item DO WE HAVE TO CHOOSE $\tau$ FOR EACH VALUE OF $\sigma_v$?
%  \item IT SEEMS THAT CHANGING $\sgm_2$ and $\tau$ BY THE SAME FACTOR LEAVES THE RESULTS IDENTICAL. INTERESTING.
%\end{enumerate}

%\section{Target Tracking Applications}\label{section:tracking}
%In this section we consider several fundamental problems commonly met in sensor fusion and target tracking applications and show how these may be solved, without approximations, within the deterministic framework of Section~\ref{section:problem}.
%%\subsection{Dealing with Outliers}\label{section:outliers}
%\subsection{Fixed-Lag Smoothing}\label{section:smoothing}

\section{Applications}\label{section:applications}
In this section we consider several classical applications commonly addressed in the Bayesian manner and show how these can be treated with the considered deterministic framework.
\subsection{Prediction}\label{section:prediction}
In order to derive optimal, in the sense of Section~\ref{section:derivation}, predictor we consider Eqs.~\ref{Eq:recursive:estimator:d:extra} and~\ref{Eq:recursive:covariance:d:extra} such that $m$ is some index representing $t_m$ at which $\hat{x}_m$ and $P_m$ are known and $k$ is an index representing some future time $t_k\triangleq t_m+\Delta$. It is assumed that no additional informative measurements are available for the computation of $\hat{x}_k$. This is equivalent to setting infinite covariance to any new measurement thus nullifying the second summand in Eqs.~\ref{Eq:recursive:estimator:d:extra} and~\ref{Eq:recursive:covariance:d:extra} which then become
\begin{align}\label{Eq:recursive:estimator:prediction}
\hat{x}_k
&=A_{k,m}\hat{x}_{m}\\\label{Eq:recursive:covariance:prediction}
P_k&=\tfrac{1}{W_{m,k}^2}A_{k,m}P_{m}A_{k,m}^T.
\end{align}
Note that the state prediction equation is exactly the same as in the KF case and the difference in the covariance expression is along the lines of the discussion in Section~\ref{section:wif:kalman}.
\subsection{Smoothing}\label{section:smoothing}
Some smoothing problems are trivially obtained from Eqs.~\ref{Eq:recursive:estimator:d:extra} and~\ref{Eq:recursive:covariance:d:extra}. For example, for fixed point smoothing we simply set $m=k$ in which case $W_{m,k}=1$ and $A_{m,k}=I$. The resulting equations implement the smoothing scheme for the state $x_k$ using the relevant measurements. Fixed-lag smoothing is obtained similarly by considering a constant lag ${t_k-t_m}$ in the above equations.
%\subsubsection{Fixed-Point Smoothing}\label{section:fixed:point}
%YYY
%The Deterministic property make the estimation optimal for any time $t_m$ and not only for $t_k$ . This property blurs the diffrence between estimation, smoothing and prediction. In our case, the only diffrence between those options determind by $dt$ and there for can be obtain easily from~\eqref{Eq:recursive:estimator:wif} and~\eqref{Eq:recursive:covariance:wif}
%\begin{align}\label{Eq:information:smoother:state}
%\hat{x}_{k+dt}
%&=A_{dt}\hat{x}_{k}
%\end{align}
%where $P_{k+dt}$ is given by
%\begin{align}\label{Eq:information:smoother:covariance}
%P_{k+dt}=A_{dt}P_kA_{dt}^T
%\end{align}
%While negative $dt$ means smoothing  and positive $dt$ mean prediction and
%\begin{align}\label{Eq:information:transion}
%A_{dt}=A_{k+dt,k}
%\end{align}
%SSS
%\subsubsection{Fixed-Lag Smoothing}\label{section:fixed:lag}
%\subsubsection{Fixed-Interval Smoothing}\label{section:fixed:interval}
\subsection{Out-of-Sequence Measurement Processing}\label{section:oosm}
In centralized multisensor fusion systems, measurements acquired at different sensors are transmitted to the fusion center, at which they are processed by a tracking filter. For example, in an aided navigation system, inertial errors are being compensated by a navigation filter fed by measurements from some external source, e.g., GPS. Typically, measurements originating at the same sensor arrive at the fusion center in the order they have been generated, that is, in-sequence. However, such synchronization does not necessarily hold for measurements acquired by different sensors due to, e.g, inevitable communication delays. Thus, it is common practice that measurements arrive ``out-of-sequence'', namely, some may arrive after other measurements, having later time-tags, have already been processed. Whereas the simplest suboptimal solution would be discarding measurements with time-tags from the past, the most computationally expensive, yet optimal approach is to reprocess the measurements in the correct order upon an OOSM is acquired. In the Bayesian setup there are simple cases in which optimality may be preserved while maintaining moderate computational requirements~\cite{ybs:2002:oosm}. A suboptimal variant for a more general setup was proposed in~\cite{ybs:2004:oosm:multistep}. The main challenge in utilizing out-of-sequence measurements in the Bayesian setup is the correlation generated by the past measurements and the process noise sequence. Significant effort has been done to treat OOSM. Some recent contributions, in addition to those cited above, include~\cite{koch:2011:oosm:accumulated},~\cite{zhang2012optimal} and references therein. In all cases, a significant modification of the original Kalman filter is required in order to cope with OOSM in either exact or approximate manner.

In the sequel we demonstrate how the OOSM utilization may be done in a simple manner using the EWIF approach.
First, we rewrite Eqs.~\eqref{Eq:recursive:estimator:d} and~\eqref{Eq:recursive:covariance:d} using the weighting function~\eqref{Eq:recursive:W2}.
\begin{align}\label{Eq:recursive:estimator:d:oosm}
\hat{x}_k
&=P_k\big(e^{-\frac{t_k-t_{k-1}}{\tau}}A_{k-1,k}^TP_{k-1}^{-1}\hat{x}_{k-1}
+e^{-\frac{t_k-t_{d}}{\tau}}A_{d,k}^TH_d^TR_d^{-1}y_{d}\big),
\end{align}
where the estimator covariance, $P_k$, is given by
\begin{align}\label{Eq:recursive:covariance:d:oosm}
P_k^{-1}
&=e^{-\frac{t_k-t_{k-1}}{\tau}}A_{k-1,k}^TP_{k-1}^{-1}A_{k-1,k}
+e^{-\frac{t_k-t_{d}}{\tau}}A_{d,k}^TH_d^TR_d^{-1}H_dA_{d,k}.
\end{align}
Recall that here $t_k$ is the time at which the state update is required, which is also the time at which the current measurement is acquired, $t_{k-1}$ is the time of the previous update, and $t_d=t_{\ell_k}$ is the time for which the currently acquired measurement, $y_{\ell_k}\equiv y_d$, is valid. If $y_{\ell_k}$ is an in-sequence measurement, namely, $t_d=t_k$, then $e^{-\frac{t_k-t_{d}}{\tau}}=1$ and the update rule reduces to that of Eq.~\eqref{Eq:recursive:estimator}. If $t_d\neq t_k$ then the contribution of $y_{\ell_k}$ is reduced by an exponential factor accounting for the temporal distance of $y_{\ell_k}$ from the current time.

In order to demonstrate the algorithm for OOSM, we consider the same example as in Section~\ref{section:wif:toy}. In the present setup, however, the sinusoidal signal is observed by an additional channel with $\sigma_{v_2}=0.2$ the measurements of which undergo a delay of $0.2$ (sec). In addition, the state vector is taken to be three-dimensional comprising position, velocity and acceleration of the target, and the constant $\tau$ is taken to be $1$. The performance of the EWIF algorithm accompanied by the corresponding fixed-lag smoother is presented in Fig.~\ref{fig:toy:sine:delay}.

\begin{figure}[h!]\centering
{\includegraphics[width=0.75\columnwidth, trim=0cm -0.5cm 0cm 0cm, clip]{fig2_2_new.eps}}%\hspace{0.2cm}
\caption{Tracking a sine signal in the presence of OOSM using EWIF (green line). The black curve represents the Exponentially Weighted Information (fixed-lag) Smoother (EWIS). The RMS errors of EWIF and the EWIS are, respectively, 0.12 and 0.06. Ignoring the out-of-sequence measurements (cyan pluses) increases the RMS errors of EWIF and EWIS to $0.23$ and $0.14$, respectively.}
\label{fig:toy:sine:delay}
\end{figure}

%\subsection{Track Fusion}\label{section:fusion}
%Track fusion is a fundamental problem commonly met in distributed filtering applications. The main idea is to allow local trackers generate estimates using their local measurements and then
%\cite{bar1986effect}

%\section{Numerical Study}\label{section:numerical}

\section{Concluding Remarks}\label{section:concluding}
We presented a deterministic framework for state estimation in dynamical systems. As opposed to the classical approach, where (random) process noise is used to cope with inevitable uncertainties in the dynamical model, in the presented modeling, this uncertainty is treated by assigning exponentially decaying weights to the observations, such that more recent measurements are assigned more weight than ``older'' ones. The state is then estimated using a weighted least-squares algorithm as opposed to Bayesian methods such as, e.g., Kalman filter. For the chosen weighting function, the least squares algorithm possesses a convenient recursive form similarly to the Kalman filter. While the deterministic formulation is not knew, it has, in the absence of process noise, several practical implications allowing exact solutions to problems which may be solved only approximately in the Bayesian setup. The OOSM processing is one of such problems and the utility of the EWIF approach was demonstrated in a simple numerical example.


%\section{To be Included in Final Paper}
%Several issues will be discussed in the final version of the paper. First, a complete derivation of the algorithms for sensor calibration will be provided and the algorithms will be summarized in an easy-to-implement manner. This includes both the 3D and 2D cases. Second, the convergence proof will be provided. Finally, a comprehensive numerical study including both performance analysis and robustness to the various parameters will be presented.


\appendix
\section{Appendix}
\label{appendix}
\subsection{Proof of Theorem~\ref{theorem:batch}}\label{appendix:batch}
Setting to zero the gradient of~\eqref{Eq:problem:WLS} with respect to $x_k$  we obtain
\[
\sum_{\ell\in\mathcal{L}}A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(H_\ell(A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k})-y_\ell)=0.
\]
Solving for $x_k$ yields~\eqref{Eq:batch:estimator}.
\subsection{Proof of Theorem~\ref{theorem:covariance}}\label{appendix:covariance}
Let
\begin{align}
\Sigma_k&\triangleq\paren{\sum_{\ell\in\mathcal{L}}A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^TH_\ell A_{\ell,k}}\\
\Psi_{\ell,k}&\triangleq A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^T
\end{align}
and consider the covariance of the estimator~\eqref{Eq:batch:estimator}
\begin{align}\non
P_k
&=\cov\left(\Sigma_k^{-1}\sum_{\ell\in\mathcal{L}}\Psi_{\ell,k}(y_\ell-H_\ell C_{\ell,k}u_{\ell,k})\right)\\\non
&=\Sigma_k^{-1}\paren{\sum_{\ell\in\mathcal{L}}\Psi_{\ell,k}{W}_{\ell,k}^{-T}R_\ell{W}_{\ell,k}^{-1}\Psi_{\ell,k}^T}\Sigma_k^{-T}.
\end{align}
Cancelling out appropriate terms and their inverses~\eqref{Eq:batch:covariance} follows.
\subsection{Proof of Theorem~\ref{theorem:recursive}}\label{appendix:recursive}
Consider the inverse of the covariance computed in batch form~\eqref{Eq:batch:covariance}
\begin{align}\non%\label{App:covariance:recursive}
P_k^{-1}&=\sum_{\ell=1}^kA_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^TH_\ell A_{\ell,k}\\\label{Eq:covariance:recursive:proof}
&=\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^TH_\ell A_{\ell,k}
+H_k^TR_k^{-1}H_k,
\end{align}
where we used the fact that $A_{k,k}=I$ as well as the assumption~\eqref{Eq:recursive:W:equal}. Using the fact that $A_{\ell,k}=A_{\ell,k-1}A_{k-1,k}$ as well as the assumption~\eqref{Eq:recursive:W:telescopic} the result for the covariance follows.
%&=\sum_{\ell=1}^{k-1}(A_{\ell,k-1}A_{k-1,k})^TH_\ell^TW_{k,\ell}R_\ell^{-1}W_{k,\ell}^TH_\ell(A_{\ell,k-1}A_{k-1,k})\\
%&\qquad+H_\ell^TR_\ell^{-1}H_\ell\\
%\end{align}
We utilize this result to prove the expression for $\hat{x}_k$. Consider the batch formulation first
%\begin{align}\non
%\hat{x}_k
%&=P_k\sum_{\ell=1}^kA_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(y_\ell-H_\ell C_{\ell,k}u_{\ell,k})\\\label{Eq:estimate:recursive:proof1}
%&=P_k\Big(\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}^2R_\ell^{-1}(y_\ell-H_\ell C_{\ell,k}u_{\ell,k})
%+H_k^TR_k^{-1}y_k\Big).
%\end{align}
\begin{align}\non
\hat{x}_k
&=P_k\sum_{\ell=1}^kA_{\ell,k}^TH_\ell^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^Ty_\ell\\\label{Eq:estimate:recursive:proof1}
&=P_k\Big(\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}^2R_\ell^{-1}y_\ell+H_k^TR_k^{-1}y_k\Big).
\end{align}
Consider the summation
%\begin{align}\non
%&\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}^2R_\ell^{-1}(y_\ell-H_\ell C_{\ell,k}u_{\ell,k})\\\non
%&\,=A_{k-1,k}^TW_{k-1,k}^2\sum_{\ell=1}^{k-1}A_{\ell,k-1}^TH_\ell^TW_{\ell,k-1}^2R_\ell^{-1}(y_\ell-H_\ell C_{\ell,k}u_{\ell,k}).
%\end{align}
\begin{align}\non
&\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}^2R_\ell^{-1}y_\ell
=A_{k-1,k}^TW_{k-1,k}^2\sum_{\ell=1}^{k-1}A_{\ell,k-1}^TH_\ell^TW_{\ell,k-1}^2R_\ell^{-1}y_\ell.
\end{align}
%It is easy to see that
%\[
%C_{\ell,k}u_{\ell,k}=A_{\ell,k-1}C_{k-1,k}u_{k-1,k}+C_{\ell,k-1}u_{\ell,k-1},
%\]
%which renders the above summation as follows
%\begin{align}\nonumber
%&\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}^2R_\ell^{-1}(y_\ell-H_\ell C_{\ell,k}u_{\ell,k})\\\non
%&\quad=A_{k-1,k}^TW_{k-1,k}^2\sum_{\ell=1}^{k-1}A_{\ell,k-1}^TH_\ell^TW_{\ell,k-1}^2R_\ell^{-1}\\\non
%&\qquad\times(y_\ell-H_\ell (A_{\ell,k-1}C_{k-1,k}u_{k-1,k}+C_{\ell,k-1}u_{\ell,k-1})).
%\end{align}
%The latter becomes, using~\eqref{Eq:batch:estimator} and~\eqref{Eq:batch:covariance},
%\begin{align}\nonumber
%&\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}^2R_\ell^{-1}(y_\ell-H_\ell C_{\ell,k}u_{\ell,k})\\\non
%&\quad=A_{k-1,k}^TW_{k-1,k}^2P_{k-1}^{-1}\hat{x}_{k-1}\\\non
%&\qquad\qquad-A_{k-1,k}^TW_{k-1,k}^2P_{k-1}^{-1}C_{k,k-1}u_{k,k-1}.
%%\\\non &\quad=A_{k-1,k}^TW_{k-1,k}^2P_{k-1}^{-1}(\hat{x}_{k-1}-C_{k,k-1}u_{k,k-1}).
%\end{align}
Using~\eqref{Eq:batch:estimator} and~\eqref{Eq:batch:covariance} the latter becomes
\begin{align}
&\sum_{\ell=1}^{k-1}A_{\ell,k}^TH_\ell^TW_{\ell,k}^2R_\ell^{-1}y_\ell
=A_{k-1,k}^TW_{k-1,k}^2P_{k-1}^{-1}\hat{x}_{k-1}.
%\\\non &\quad=A_{k-1,k}^TW_{k-1,k}^2P_{k-1}^{-1}(\hat{x}_{k-1}-C_{k,k-1}u_{k,k-1}).
\end{align}
Plugging this result in~\eqref{Eq:estimate:recursive:proof1} completes the proof.



\subsection{Proof of Theorem~\ref{theorem:efficient}}\label{appendix:efficient}
The unbiasedness follows trivially by substituting~\eqref{Eq:problem:state} in~\eqref{Eq:problem:measurement}, plugging the result in~\eqref{Eq:batch:estimator} and taking mathematical expectation. In order to show that the estimator is efficient we compute the Fisher information matrix corresponding to~\eqref{Eq:problem:measurement2}. To this end, we consider
$p(x_k\mid y_\ell,\,\ell\in\mathcal{L})$ -- the likelihood function of $x_k$ given the set of measurements $\set{y_\ell,\,\ell\in\mathcal{L}}$.
Recalling~\eqref{Eq:problem:measurement2} we note that the likelihood of $x_k$ given a single measurement $y_\ell$ is Gaussian with mean
%$H_\ell(A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k})$
$H_\ell A_{\ell,k}x_k$
and covariance ${W}_{\ell,k}^{-T}R_\ell{W}_{\ell,k}^{-1}$. Since the measurement noise is white, the likelihood, given the set of measurements $\set{y_\ell,\,\ell\in\mathcal{L}}$, is given by the product
%\begin{align}\non
%&p(x_k\mid y_1,\ldots,y_{\size{\mathcal{L}}})\\\label{Eq:appendix:efficient:likelihood}
%&\quad=\prod_{\ell\in\mathcal{L}}\mathcal{N}(y_\ell;H_\ell(A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k}),{W}_{\ell,k}^{-T}R_\ell{W}_{\ell,k}^{-1}),
%\end{align}
\begin{align}\label{Eq:appendix:efficient:likelihood}
&p(x_k\mid y_\ell,\,\ell\in\mathcal{L})
=\prod_{\ell\in\mathcal{L}}\mathcal{N}(y_\ell;H_\ell A_{\ell,k}x_k,{W}_{\ell,k}^{-T}R_\ell{W}_{\ell,k}^{-1}),
\end{align}
where $\mathcal{N}(y;\mu,\Sigma)$ is a Gaussian density function with mean $\mu$ and covariance matrix $\Sigma$ evaluated at $y$. The log-likelihood thus reads
%\begin{align}\non
%&\log p(x_k\mid y_1,\ldots,y_{\size{\mathcal{L}}})\\\label{Eq:appendix:efficient:loglikelihood}
%&\quad=C-\sum_{\ell\in\mathcal{L}}(H_\ell(A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k})-y_\ell)^T\\
%&\qquad \times W_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(H_\ell(A_{\ell,k}x_k+C_{\ell,k}u_{\ell,k})-y_\ell)
%\end{align}
\begin{align}\non
&\log p(x_k\mid y_\ell,\,\ell\in\mathcal{L})\\\label{Eq:appendix:efficient:loglikelihood}
&\quad=C-\sum_{\ell\in\mathcal{L}}(H_\ell A_{\ell,k}x_k-y_\ell)^TW_{\ell,k}R_\ell^{-1}W_{\ell,k}^T(H_\ell A_{\ell,k}x_k-y_\ell)
\end{align}
where $C$ is some constant that does not depend on $x_k$. Differentiating the latter twice with respect to $x_k$ yields, up to the minus sign, the inverse of~\eqref{theorem:covariance} meaning that the covariance of the estimator attains the Cram\'{e}r-Rao lower bound with equality rendering the estimator efficient.

\subsection{Proof of Lemma~\ref{lemma:scaling}}\label{appendix:scaling}
Suppose that the actual measurement noise covariance, $R_\ell$, is only known up to a constant factor $\alpha>0$ such that the value used in the algorithm is $\tilde{R}_\ell\triangleq\alpha{R}_\ell$. Plugging $\tilde{R}_\ell$ in~\eqref{Eq:batch:estimator}, it is readily seen that $\alpha$ cancels out, meaning that the imprecisely known covariance does not alter the estimator. This property is valid due to the lack of the process noise covariance term in the filter equation and cannot hold in the KF setup. We note that the covariance of the estimator, given in~\eqref{Eq:batch:covariance}, \emph{is} sensitive to the actual value of ${R}_\ell$.


\endinput


